Faster Relational Algorithms Using Geometric Data Structures

Optimization tasks over relational data, such as clustering, often suffer from the prohibitive cost of join operations, which are necessary to access the full dataset. While geometric data structures like BBD trees yield fast approximation algorithms in the standard computational setting, their application to relational data remains unclear due to the size of the join output. In this paper, we introduce a framework that leverages geometric insights to design faster algorithms when the data is stored as the results of a join query in a relational database. Our core contribution is the development of the RBBD tree, a randomized variant of the BBD tree tailored for relational settings. Instead of completely constructing the RBBD tree, by leveraging efficient sampling and counting techniques over relational joins, we enable on-the-fly efficient expansion of the RBBD tree, maintaining only the necessary parts. This allows us to simulate geometric query procedures without materializing the join result. As an application, we present algorithms that improve the state-of-the-art for relational $k$-center/means/median clustering by a factor of $k$ in running time while maintaining the same approximation guarantees. Our method is general and can be applied to various optimization problems in the relational setting.

==> covering.tex <==
\section{Other covering problems}

==> dataStructures_old.tex <==
\section{Relational Procedures Following Geometric Structures}
In this section, we design relational algorithms for some geometric tasks that will be useful in the next sections. In particular, we consider the following dynamic tasks.
\newcommand{\ball}{\mathcal{B}}
\newcommand{\cent}{c}
\newcommand{\radius}{r}
\begin{comment}
\begin{enumerate}
    \item Given $k$ balls $\ball_1(\cent_1,\radius_1),\ldots, \ball_k(\cent_1,\radius_1) \in \Re^{d}$, return a join result uniformly at random among $\Q(\I)\setminus (\bigcup_{\ell=[k]}\ball_\ell(\cent_\ell,\radius_\ell))$.
     \item Given $k$ balls $\ball_1(\cent_1,\radius_1),\ldots, \ball_k(\cent_1,\radius_1) \in \Re^{d}$, return $|\Q(\I)\cap (\bigcup_{\ell=[k]}\ball_\ell(\cent_\ell,\radius_\ell))|$.
\end{enumerate}
\end{comment}
%We will consider the following dynamic tasks.

Let $\ball_\tau(\cent_\tau,\radius_\tau)$ be a new ball that we get in the $\tau$-th timestamp and let $k$ be a parameter that denotes the maximum timestamp.
\begin{enumerate}
    \item For every timestamp $\tau\in [k]$, return a join result among $\Q(\I)\setminus (\bigcup_{\ell=[\tau]}\ball_\ell(\cent_\ell,\radius_\ell))$. For this task, instead of returning any join results out of the union of the given balls, we might want to sample uniformly at random a join result among $\Q(\I)\setminus (\bigcup_{\ell=[\tau]}\ball_\ell(\cent_\ell,\radius_\ell))$.

    \item For every timestamp $\tau=[k]$, return $|\Q(\I)\cap (\bigcup_{\ell=[\tau]}\ball_\ell(\cent_\ell,\radius_\ell))|$.
\end{enumerate}
Our goal is to design algorithms for both tasks that run in roughly $\O(N)$ time for every new ball $\ball_\tau$ we receive.
Such dynamic algorithms would lead to $\O(kN)$ time algorithms for i) Given $k$ balls $\ball_1(\cent_1,\radius_1),\ldots, \ball_k(\cent_k,\radius_k)$, returning a join result among $\Q(\I)\setminus (\bigcup_{\ell=[k]}\ball_\ell(\cent_\ell,\radius_\ell))$, and ii) given $k$ balls $\ball_1(\cent_1,\radius_1),\ldots, \ball_k(\cent_k,\radius_k)$, return $|\Q(\I)\cap (\bigcup_{\ell=[k]}\ball_\ell(\cent_\ell,\radius_\ell))|$.



We design efficient relational approximation algorithms for the tasks above by implicitly constructing and maintaining a geometric data structure, such that a quad tree, a bbd tree, a range tree or a kd tree.

\subsection{Quad tree}

\subsection{BBD tree}

\subsection{Range tree and kd tree}
